Neutrino Non-Standard Interactions: A Status Report

This report summarizes the present status of neutrino non-standard interactions (NSI). After a brief overview, several aspects of NSIs are discussed, including connection to neutrino mass models, model-building and phenomenology of large NSI with both light and heavy mediators, NSI phenomenology in both short- and long-baseline neutrino oscillation experiments, neutrino cross-sections, complementarity of NSI with other low- and high-energy experiments, fits with neutrino oscillation and scattering data, DUNE sensitivity to NSI, effective field theory of NSI, as well as the relevance of NSI to dark matter and cosmology. We also discuss the open questions and interesting future directions that can be pursued by the community at large. This report is based on talks and discussions during the Neutrino Theory Network NSI workshop held at Washington University in St. Louis from May 29-31, 2019 (https://indico.cern.ch/event/812851/)

==> README <==
Hello everyone,
Bhupal has made a skeleton for us to add contributions. You can look at the "example.tex" file in the "contributions" folder to see the basic structure, or read through Peter's contribution in "denton.tex".

The "main.tex" file will compile all other subfiles. Add your subsections to the main document with your titles like so:

\subsection{This is an Example Contribution Title (by Example Author)}
\subfile{contributions/example.tex}

...and then create your subfile.tex within the "contributions" folder. Currently, your citations will not appear when locally compiling each of your individual contributions, but they will appears with you click into "main.tex" and then recompile. Put everything in the "refs.bib" with appropriate formatting, I believe from iNSPIRE-HEP.

Put your figures in the "images" folder for ease of scrolling through them all, as well as referencing and including them (folders are searchable and auto-completeable in OverLeaf!)
